Domain Theory Meets Interaction Trees in Rocq

We present a domain-theoretical formalization of interaction trees in the Rocq prover. Unlike existing formalizations, ours does not rely on Rocq's built-in coinduction. Hence, we avoid complications occurring in earlier works, such as artificially including silent steps to comply with Rocq's productivity checker, treating monad laws as weak bisimulations, and coinductive bisimulation reasoning. We define an inductive program equivalence relation as the congruence closure of a base relation on primitive effects with respect to action sequencing and least upper bounds. This enables reasoning about possibly non-terminating programs by reducing their equivalences to equivalences of their terminating approximations, which are then proved by induction. This relation is proved correct: provided the base relation is correct, equivalent computations have equal denotations in any monad that faithfully implements the effects. We illustrate the framework by showing the equivalence of two programs encoding the Syracuse sequence, whose termination is an open mathematical conjecture.

==> eptcsdata.tex <==
\providecommand{\firstpage}{122}
\providecommand{\publicationstatus}{Mircea Marin, Adrian Cr\u{a}ciun (Eds.): FROM 2026\\
EPTCS 452, 2026, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.452.9}{10.4204/EPTCS.452.9}}

